MuCoS: Efficient Drug Target Discovery via Multi Context Aware Sampling in Knowledge Graphs

Accurate prediction of drug target interactions is critical for accelerating drug discovery and elucidating complex biological mechanisms. In this work, we frame drug target prediction as a link prediction task on heterogeneous biomedical knowledge graphs (KG) that integrate drugs, proteins, diseases, pathways, and other relevant entities. Conventional KG embedding methods such as TransE and ComplEx SE are hindered by their reliance on computationally intensive negative sampling and their limited generalization to unseen drug target pairs. To address these challenges, we propose Multi Context Aware Sampling (MuCoS), a novel framework that prioritizes high-density neighbours to capture salient structural patterns and integrates these with contextual embeddings derived from BERT. By unifying structural and textual modalities and selectively sampling highly informative patterns, MuCoS circumvents the need for negative sampling, significantly reducing computational overhead while enhancing predictive accuracy for novel drug target associations and drug targets. Extensive experiments on the KEGG50k dataset demonstrate that MuCoS outperforms state-of-the-art baselines, achieving up to a 13\% improvement in mean reciprocal rank (MRR) in predicting any relation in the dataset and a 6\% improvement in dedicated drug target relation prediction.

==> commented_out.tex <==
\begin{abstract}
%Drug-target interactions are critical for understanding biological processes and advancing drug discovery. However, traditional methods such as ComplEx-SE, TransE, and DistMult struggle with unseen relationships and negative triplets, which limits their effectiveness in drug-target prediction. To address these challenges, we propose Multi-Context-Aware Sampling (MuCoS), an efficient and positively accurate method for drug-target prediction. MuCoS reduces computational complexity by prioritizing neighbors of higher density to capture informative structural patterns. These optimized neighborhood representations are integrated with BERT, enabling contextualized embeddings for accurate prediction of missing relationships or tail entities. MuCoS avoids the need for negative triplet sampling, reducing computation while improving performance over unseen entities and relations. Experiments on the KEGG50k biomedical dataset show that MuCoS improved over existing models by 13\% on MRR, 7\% on Hits@1, 4\% on Hits@3, and 18\% on Hits@10 for the general relationship, and by 6\% on MRR, 1\% on Hits@1, 3\% on Hits@3, and 12\% on Hits@10 for prediction of drug-target relationship.
\end{abstract}



\section{Related Work}
%Similarity-based DTI prediction methods utilize drug and target similarity measures in conjunction with the distance between each pair of drugs and their respective targets \cite{shi2018drug}. The similarity is obtained using a distance function like the Euclidean.
%The DTI prediction using feature-based approaches uses mainly the support vector machine \cite{zhang2017drugrpe}. A pair of targets and drugs can be distinguished by features, leading to binary classification or two-class clustering based on positive or negative relations.
%Currently, graph-based approaches used in parallel with network-based methods to predict missing DTI are considered reliable relations prediction methods \cite{ban2019nrlmfbeta}. Here, drug-drug similarity, target-target similarity, and known relations between DTI are integrated into a heterogeneous network, operating on the simple logical principle that similar drugs interact with similar targets.

%Embedding-based approaches (KGE) such as TransE \cite{bordes2013translating} and RotatE \cite{sun2019rotate} incorporate the fundamental semantics of a graph by expressing entities and relationships between them as continuous vectors. In contrast, semantic or textual matching techniques such as DistMult \cite{yang2014embedding}, utilize scoring functions to evaluate the similarity of entities and relationships. By looking at the scores for all the relationships and entities linked to a certain head/tail and relationship, these methods find the most likely relationship or tail entity during testing. 

%In summary, existing KGC methodologies exhibit notable limitations. Embedding models such as TransE, RotatE, and others fail to generalize to unseen entities and relations because of their dependence on predefined embeddings, limiting adaptability to new structures. Text-based and LLM-based approaches depend on descriptive entity information, which is often sparse or inconsistent across datasets. In addition, embedding methods, as well as some text-based methods, rely on extensive negative sampling during training, leading to high computational costs, especially on large datasets. 


\textit{\textbf{Dataset}:} 
The proposed model was evaluated on the KEGG50k medical domain dataset, which contains 63,080 triples, split into 57,080 for training, 3,000 for validation, and 3,000 for testing. These triples represent relationships among biological entities drugs $\mathcal{E}_d$ and genes $\mathcal{E}_g$. The dataset comprises 16,201 unique entities $\mathcal{E}$ where $( \mathcal{E}_d \cup \mathcal{E}_g) \subseteq \mathcal{E}$ and 9 distinct types of drug-target relationships.
KEGG50k is a subset of the KEGG database, because it provides a robust collection of 50,000 curated drug-target relations and genes, enabling efficient evaluation of MuCoS's ability to predict high-density contextual relationships in pharmaceutical research. This dataset is important for finding new drug targets and genes because it includes molecular pathways and interaction networks that are needed to find therapeutic targets that are biologically relevant.


\textit{\textbf{Task (1) - Relationship Prediction}}: The experimental results in Table \ref{tab:link_prediction} highlight the effectiveness of our proposed MuCoS methodology for both general and drug-target relationship prediction tasks on the KEGG50k dataset. Notably, MuCoS achieves a Mean Reciprocal Rank (MRR) of 0.65 for general link prediction, a 13\% improvement over the previous best-performing model, ComplEx-SE (MRR of 0.52). Its Hits@1 score of 0.52 surpasses ComplEx-SE’s 0.45 by 7\%, demonstrating MuCoS’s ability to rank relationships accurately as the top prediction. Additionally, Hits@3 and Hits@10 scores of 0.60 and 0.86, respectively, further underscore MuCoS’s robustness, outperforming other baseline models significantly.
